Technical Report -- Expected Exploitability: Predicting the Development of Functional Vulnerability Exploits

Assessing the exploitability of software vulnerabilities at the time of disclosure is difficult and error-prone, as features extracted via technical analysis by existing metrics are poor predictors for exploit development. Moreover, exploitability assessments suffer from a class bias because "not exploitable" labels could be inaccurate. To overcome these challenges, we propose a new metric, called Expected Exploitability (EE), which reflects, over time, the likelihood that functional exploits will be developed. Key to our solution is a time-varying view of exploitability, a departure from existing metrics. This allows us to learn EE using data-driven techniques from artifacts published after disclosure, such as technical write-ups and proof-of-concept exploits, for which we design novel feature sets. This view also allows us to investigate the effect of the label biases on the classifiers. We characterize the noise-generating process for exploit prediction, showing that our problem is subject to the most challenging type of label noise, and propose techniques to learn EE in the presence of noise. On a dataset of 103,137 vulnerabilities, we show that EE increases precision from 49% to 86% over existing metrics, including two state-of-the-art exploit classifiers, while its precision substantially improves over time. We also highlight the practical utility of EE for predicting imminent exploits and prioritizing critical vulnerabilities. We develop EE into an online platform which is publicly available at https://exploitability.app/.

==> discussion.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% discussion.tex  --
%  
%   Discussion.
%
% !TEX root = functional_exploits.tex
% Last modified:		$Date:: 2019-09-14 #$  by   $Author: osuciu $
% SVN revision:   	$Rev: 7497 $
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\section{Discussion}
\label{sec:discussion}
\todo{revise and re-write}
%After performing a large scale analysis of the utility of PoCs for predicting exploits, in this section we discuss the implications of our results for the security community.
Below we discuss the broader implications of our results for the security community.

\topic{Exploitability as a time-varying function}\todo{cut this since we have it in the problem statmeent} The Exploit Code Maturity component of the Temporal CVSS score, which is designed to track the real-time exploit availability, is not updated in NVD.
The default "Not defined" translates to the highest severity assessment, which means that the majority of vulnerabilities receivie the highest severity score by default.
However, as our results indicate that fewer than 25\% of vulnerabilities actually get exploited, the severity of the majority would get over-estimated.
While the temporal score is available in third-party databases like IBM X-Force~\cite{xforce} and Tenable Nessus~\cite{Tenable:Nessus}, we observed that their coverage is limited, as tracking and updating these values requires manual efforts. 
In contrast, as illustrated in Figure~\ref{fig:perf_1days_b}, our predictor can automatically improve its predictions over time, with the emergence of more information about the vulnerabilities and exploits.
%
Moreover, recent game-theoretic results about the evolution of attack strategies in cyber-warfare suggest that a time-varying view of exploitability is key to selecting the best strategy~\cite{bao2017shall}.

\topic{Expected exploitability as a prioritization tool} Our results indicate that the information from PoCs provides timely and precise assessments of the likelihood of exploitation. 
Based on this observation, our tool can be applied as an addition to existing vulnerability management and prioritization products~\cite{Tenable:IO}, allowing them to directly combine our dynamic estimates with other static metrics, such as the CVSS score.
Moreover, the tool could also prove useful in the cyber-insurance industry~\cite{bohme2010modeling}, where the time-varying predictions can serve as a factor for the computation of risk formulas.

\topic{Aiding exploit generation} Our technique is useful to exploit researchers who aim to assess exploitability.
Researchers aiming to generate functional exploits from PoCs can leverage our feature utility assessments to discover the PoCs which are most likely to aid exploit development.
For example, an Automated Exploit Generation (AEG) tool like FUZE~\cite{wu2018fuze} relies on high quality PoCs as seeds for exploit generation.
Nevertheless, a manual seed selection approach is subjective and could prevent the fuzzer from prioritizing the most exploitable vulnerabilities.
In contrast, a seed selection based on data-driven assessments about the PoC utility, provided by our system, can help improve the effectiveness of AEG techniques.

\topic{Timing the publication of PoCs}
Responsible disclosure policies advise participants to delay the publication of PoC by 30 days after disclosure~\cite{responsible-disclosure}, to facilitate patch deployment before they could be leveraged by attacks in the wild.
Nevertheless, our results indicate that a significant fraction of PoCs are released at or soon after disclosure.
On several instances, pubished PoCs were found to directly cause exploitation in the wild soon after disclosure~\cite{bleepingcomp-ekits,sysopfb-coblnt,zenet-phpbug}, suggesting that the manual assessments of PoC utility towards exploit development are not always accurate.
In contrast, parties could use our tool for more educated publication decisions, by observing how the exploitation likelihood would change if the PoC were to become available. 


\todo{utility for vendors as an additional tool for computing exploitability, since many PoCs are privately avialable}
\todo{functional exploits vs pocs vs exploits in the wild. decoupling the factors }
\todo{the importance of information sharing and aggregation from multiple sources for better and more timely prediction}
\todo{utility of PoCs in understanding the exploitability, since we observed interesting stuff in the keywords, complexity and tokens. reference FUZE for an early attempt and talk about AEG.}

\TODO{How easy would it be for an adversary to evade our system? -- use robust adversarial training, validate the PoCs for its effectiveness}

\todo{tool used by sysadmins to prioritize remediation. }


\TODO{Exploitability should be temporal. Why? Because it affects strategies, e.g. in CGC. , 
The Exploit Code Maturity score in the Temporal component of CVSS intended to track the real-time exploit availability, but in NVD it only has the default value -- not defined -- which overestimates the exploitability. It is populated in IBM X-Force and Tenable Nessus, but the coverage is spotty. This is because it would require manual effort. Our predictor can do this automatically, e.g. in Figure~\ref{fig:perf_1days_b} it shows that the prediction improves over time, as we get more information about the exploits.}

\todo{tool used by exploit researchers to prioritize exploit development.}


==> numbers.tex <==
%--------------------------------------------------------------------------
% Numbers that must be quoted consistently throughout the paper
%\newcommand{\ApplicationsSelected}[0]{10\xspace}
%\newcommand{\HostsWINEMillions}[0]{8.4\xspace}
%\newcommand{\FilesWINE}[0]{7,196,952\xspace}
%\newcommand{\FilesWINEMillions}[0]{7.1\xspace}
%\newcommand{\ExploitsWINEAV}[0]{244\xspace}
%\newcommand{\FilesVT}[0]{5,194,029\xspace}
%\newcommand{\FilesVTMillions}[0]{5.1\xspace}
%\newcommand{\NVDVuls}[0]{59,875\xspace}
%\newcommand{\NVDVulsThousands}[0]{59\xspace}
%\newcommand{\OSVDBVuls}[0]{77,101\xspace}
%\newcommand{\OSVDBVulsThousands}[0]{77\xspace}
%\newcommand{\EDBExploits}[0]{25,331\xspace}
%\newcommand{\EDBExploitsThousands}[0]{25\xspace}
%\newcommand{\VulnerabilitiesSelected}[0]{1,593\xspace}
%\newcommand{\VulnerabilityClusters}[0]{408\xspace}		% only 397 in the survival data
%\newcommand{\VulnerabilitiesPerCluster}[0]{3.9\xspace}
%\newcommand{\ObservationPeriodLengthYears}[0]{5\xspace}
%
%
%\newcommand{\SoPWeekBeforeAfter}[0]{77\%\xspace}
%\newcommand{\SoPMonthBeforeAfter}[0]{92\%\xspace}
%\newcommand{\MedianTimeToPatchVulnPrctReached}[0]{87\%\xspace}
%\newcommand{\MedianTimeToPatchClustPrctReached}[0]{78\%\xspace}
%\newcommand{\MedianTimeToPatchMin}[0]{0\xspace}
%\newcommand{\MedianTimeToPatchMax}[0]{1156\xspace}
%\newcommand{\MedianTimeToPatchMedian}[0]{45\xspace}
%\newcommand{\MedianTimeToPatchAverage}[0]{101\xspace}
%\newcommand{\NinetyfiveTimeToPatchVulnPrctReached}[0]{28\%\xspace}
%\newcommand{\NinetyfiveTimeToPatchClustPrctReached}[0]{26\%\xspace}
%\newcommand{\NinetyfiveTimeToPatchMin}[0]{0\xspace}
%\newcommand{\NinetyfiveTimeToPatchMax}[0]{1452\xspace}
%\newcommand{\NinetyfiveTimeToPatchMedian}[0]{429\xspace}
%\newcommand{\NinetyfiveTimeToPatchAverage}[0]{434\xspace}
%\newcommand{\ExploitsMatchedWINE}[0]{13\xspace}		% 11 distinct CVEs (some CVEs affect more than one app)
%\newcommand{\ExploitsMatchedEDB}[0]{50\xspace}		% 46 distinct CVEs
%\newcommand{\ExploitsMatchedAll}[0]{54\xspace}		% 50 distinct CVEs
%\newcommand{\VulnerabilitySurvivalAtExploitationMedian}{86\%\xspace}
%\newcommand{\PatchLevelAtExploitationMedian}{14\%\xspace}
%\newcommand{\PatchCompletionCutoff}[0]{98.7\%\xspace}
%\newcommand{\PatchCompletionVulnerabilities}[0]{30\xspace}
%\newcommand{\PatchCompletionHalfTimeMeanClusters}[0]{213 days\xspace}  % 213.4749035
%--------------------------------------------------------------------------

\newcommand{\problem}[0]{expected exploitability\xspace}
